How to Model Brushless Electric Motors for the Design of Lightweight Robotic Systems

A key step in the development of lightweight, high performance robotic systems is the modeling and selection of permanent magnet brushless direct current (BLDC) electric motors. Typical modeling analyses are completed a priori, and provide insight for properly sizing a motor for an application, specifying the required operating voltage and current, as well as assessing the thermal response and other design attributes (e.g.transmission ratio). However, to perform these modeling analyses, proper information about the motor's characteristics are needed, which are often obtained from manufacturer datasheets. Through our own experience and communications with manufacturers, we have noticed a lack of clarity and standardization in modeling BLDC motors, compounded by vague or inconsistent terminology used in motor datasheets. The purpose of this tutorial is to concisely describe the governing equations for BLDC motor analyses used in the design process, as well as highlight potential errors that can arise from incorrect usage. We present a power-invariant conversion from phase and line-to-line reference frames to a familiar q-axis DC motor representation, which provides a ``brushed'' analogue of a three phase BLDC motor that is convenient for analysis and design. We highlight potential errors including incorrect calculations of winding resistive heat loss, improper estimation of motor torque via the motor's torque constant, and incorrect estimation of the required bus voltage or resulting angular velocity limitations. A unified and condensed set of governing equations is available for designers in the Appendix. The intent of this work is to provide a consolidated mathematical foundation for modeling BLDC motors that addresses existing confusion and fosters high performance designs of future robotic systems.

==> Unused/unused.tex <==
% %% for duplicating table control sequence
 \definecollection{mytable}
 \definecollection{kvtable}
\newcounter{duptable}
\newcounter{tmp}
\newcounter{kvduptable}
\newcounter{kvtmp}

\makeatletter
\newcommand\resttable{%
\let\oldlabel\label
\let\label\@gobble
\setcounter{tmp}{\value{table}}
\setcounter{table}{\value{duptable}}
\includecollection{mytable}
\let\label\oldlabel
\setcounter{table}{\value{tmp}}
}
\newcommand\resttablekv{%
\let\oldlabel\label
\let\label\@gobble
\setcounter{kvtmp}{\value{table}}
\setcounter{table}{\value{kvduptable}}
\includecollection{kvtable}
\let\label\oldlabel
\setcounter{table}{\value{kvtmp}}
}
\makeatother

% The maximum torque that a motor can produce at a certain current can be estimated by \ref{eq:kt_q}, but many manufacturers do not provide the torque constant with respect to the q-axis current. (\ref{eq:kt_wye}) and (\ref{eq:kt_delta}) can be used to convert torque constants from given frames of reference to q-axis representation.
% \begin{align}
% \text{Wye:}&\;\;\;\;\;\;\;K_t^q = \sqrt{\frac{3}{2}} K_t^{\phi} = \sqrt{3} K_t^{rms} = \sqrt{\frac{2}{3}} K_t^{L} \label{eq:kt_wye}\\
% \text{Delta:}&\;\;\;\;\;\;\;K_t^q = \sqrt{\frac{3}{2}} K_t^{\phi} = \sqrt{3} K_t^{rms} = \sqrt{2} K_t^{L} \label{eq:kt_delta}
% \end{align}
% To convert torque constants with a given frame of reference, equation \ref{eq:conversion_kt} can be used with the appropriate conversion factor listed in Table \ref{tab:conversions_kt}:
%  \begin{equation} \label{eq:conversion_kt}
%      k_t^q = c \cdot k_t^{other}
%  \end{equation}

% \begin{collect*}{mytable}{\setcounter{duptable}{\value{table}}}{}{}{}
%  \begin{table}[h]
%      \centering
%      \begin{tabular}{c|c|c}
%      \hline
%      $k_t$ given w.r.t. &Delta&Wye \\
%      \hline
%      $I^q$ & 1 & 1 \\
%      $I^{\phi}$ & $\sqrt{\frac{3}{2}}$ & $\sqrt{\frac{3}{2}}$ \\
%      $I^{rms}$ & $\sqrt{3}$ & $\sqrt{3}$ \\
%      $I^{L}$ & $\sqrt{2}$ & $\sqrt{\frac{2}{3}}$
%      \end{tabular}
%      \caption{Conversion factor $c$ for common torque constant representations}
%      \label{tab:conversions_kt}
%  \end{table}
%  \end{collect*}
% wrong combinations of Kt and I resulting in instantaneous torque estimation
